Selective Classification Under Distribution Shifts

In selective classification (SC), a classifier abstains from making predictions that are likely to be wrong to avoid excessive errors. To deploy imperfect classifiers -- either due to intrinsic statistical noise of data or for robustness issue of the classifier or beyond -- in high-stakes scenarios, SC appears to be an attractive and necessary path to follow. Despite decades of research in SC, most previous SC methods still focus on the ideal statistical setting only, i.e., the data distribution at deployment is the same as that of training, although practical data can come from the wild. To bridge this gap, in this paper, we propose an SC framework that takes into account distribution shifts, termed generalized selective classification, that covers label-shifted (or out-of-distribution) and covariate-shifted samples, in addition to typical in-distribution samples, the first of its kind in the SC literature. We focus on non-training-based confidence-score functions for generalized SC on deep learning (DL) classifiers, and propose two novel margin-based score functions. Through extensive analysis and experiments, we show that our proposed score functions are more effective and reliable than the existing ones for generalized SC on a variety of classification tasks and DL classifiers. Code is available at https://github.com/sun-umn/sc_with_distshift.

==> Figure-Tex/Cifar-10-RC-Curves.tex <==
\begin{figure}[!tb]
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{cccc}
\centering
\includegraphics[width=0.21\textwidth]{Figures/Cifar10-Vit/RC-Curves/Clean-RC-Curve.png}%
&\includegraphics[width=0.21\textwidth]{Figures/Cifar10-Vit/RC-Curves/gaussian_blur_1.png}%
&\includegraphics[width=0.21\textwidth]{Figures/Cifar10-Vit/RC-Curves/gaussian_blur_3.png}%
&\includegraphics[width=0.21\textwidth]{Figures/Cifar10-Vit/RC-Curves/gaussian_blur_5.png}%
\\
{\textbf{(a)} CIFAR-10 (clean)}%
&{\textbf{(b)} Gaussian blur Lv.1}%
&{\textbf{(c)} Gaussian blur Lv.3}%
&{\textbf{(d)} Gaussian blur Lv.5}%
\end{tabular}}%
\caption{RC curves achieved by different selection confidence on \textbf{(a)} CIFAR-10, \textbf{(b)-(d)} CIFAR-10-C with Guassian blur corruptions at severity $1$, $3$ and $5$, respectively. Despite that $s_{\text{ml}}$ is clearly worse, other scores result in comparable RC curves regardless the perturbation severity for this selected DNN classifier.}
\label{Fig: Cifar10 RC curves}
\vspace{-0.5em}
\end{figure}%

==> Figure-Tex/ImageNet-Cifar-Logit-Scale-Compare.tex <==
\begin{figure}[!tb]
\centering
\resizebox{0.45\columnwidth}{!}{%
\begin{tabular}{c}
{\includegraphics[width=0.24\textwidth]{Figures/Demo/Logit-Scale-Compare.png}}%
\end{tabular}\hfill
\begin{minipage}{0.2\textwidth}%
\vspace{1.5em}
\caption{Histogram of the top2 logit difference (x-axis) of the model \textbf{EVA} (evaluted on IN validation dataset) and CIFAR-10 model (evaluated on CIFAR-10 validation set).}%
\label{Fig: Logit Scale Comparison}
\end{minipage}}%
\vspace{-1em}
\end{figure}%

==> Figure-Tex/MLP-Figure-Heatmaps.tex <==
\begin{figure}[!tb]
\centering
\begingroup 
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{c c c c}
\centering

\includegraphics[width=0.24\textwidth]{Figures/MLP-Figures/Heatmap-Geo-Margin.png}
&\includegraphics[width=0.24\textwidth]{Figures/MLP-Figures/Heatmap-Max-SR.png}
&\includegraphics[width=0.24\textwidth]{Figures/MLP-Figures/Heatmap-Entropy.png}
&\includegraphics[width=0.24\textwidth]{Figures/MLP-Figures/Heatmap-Max-Logit.png}
\\
{\textbf{(a)} $s_{\text{geo}}$}
&{\textbf{(b)} $s_{\text{sr}}$}
&{\textbf{(c)} $s_{\text{h}}$}
&{\textbf{(d)} $s_{\text{ml}}$}

\end{tabular}
\endgroup 
\caption{Heat maps of different selective confidence scores within the input space (MLP classifier) --- \textbf{(a)} $s_{\text{geo}}$, \textbf{(b)} $s_{\text{sr}}$, \textbf{(c)} $s_{\text{h}}$ and \textbf{(d)} $s_{\text{ml}}$. Compared to the SVM case in \cref{Fig: Selective Confidence Heatmaps}, the patterns of different selective confidences are similar.}
\vspace{-0.5em}
\label{Fig: MLP Selective Confidence Heatmaps}
\end{figure}

==> Figure-Tex/MLP-Figure-Samples-RC.tex <==
\begin{figure}[!tb]
\vspace{-2em}
\begin{tabular}{@{}cc@{}}
    \subfloat[Visualization of samples and the MLP decision boundaries.]{%
        \includegraphics[width=0.33\textwidth]{Figures/MLP-Figures/Decision-Boundaries.png}%
    }&
    \subfloat[RC curves.]{%
        \includegraphics[width=0.33\textwidth]{Figures/MLP-Figures/RC-Curves.png}%
    }
\end{tabular}\hfill
\begin{minipage}{0.26\textwidth}
\vspace{1.5em}
\caption{Visualization of \textbf{(a)} the decision boundaries of the MLP classifier using $s_{\text{sr}}$ and $s_{\text{geo}}$ decision rules, respectively, and \textbf{(b)} the RC curves achieved by the MLP classifier paired with different selective confidence.}
\label{Fig: Vis MLP samples and RC curves}
\end{minipage}
\vspace{-0.5em}
\end{figure}

==> Figure-Tex/Partial-AURC-Demo.tex <==
% \begin{figure}[!tb]
% \centering
% \resizebox{0.4\columnwidth}{!}{%
% \begin{tabular}{c}
% {\includegraphics[width=0.21\textwidth]{Figures/Demo/AURC-alpha.png}}%
% \end{tabular}\hfill%
% \begin{minipage}{0.21\textwidth}
% \vspace{1.2em}
% \caption{Visualization of AURC-$\alpha$ (area in blue). Note that we report \emph{normalized} AURC-$\alpha$ in this paper---the blue area divided by the coverage $\alpha$.}%
% \label{Fig: Demo AURC}
% \end{minipage}}%
% \vspace{-1em}
% \end{figure}%

% \begin{figure}[!tb]
% \centering
% \begingroup 
% % \setlength{\tabcolsep}{1pt}
% % \renewcommand{\arraystretch}{0.8}
% \begin{tabular}{c c}
% \centering

% \includegraphics[width=0.21\textwidth]{Figures/Demo/AURC-alpha.png}%
% &\includegraphics[width=0.21\textwidth]{Figures/Demo/AURC-beta.png}\\
% {\textbf{(a)} AURC-$\alpha$}
% &{\textbf{(b)} AURC-$\beta$}

% \end{tabular}
% \endgroup 
% \caption{Examples of RC curves and the evaluation metrics \textbf{(i)} AURC-$\alpha$ and  \textbf{(ii)} AURC-$\beta$, where the regions in blue are the partial area under curve, and the dashed black lines are the covreage threshold $\alpha$ and risk threhsold $\beta$, respectively. Note that we use normalized AURC-$\alpha$ in this paper --- the blue area divided by $\alpha$; while we keep the raw AURC-$\beta$ values --- the corresponding $\alpha$ is always one.}
% % \vspace{-0.5em}
% \label{Fig: Demo AURC}
% \end{figure}

% \begin{figure}[!tb]
% \centering
% \includegraphics[width=0.21\textwidth]{Figures/Demo/AURC-alpha.png}%
% \caption{Visualization of AURC-$\alpha$ (area in blue). Note that we use normalized AURC-$\alpha$ in this paper --- the blue area divided by $\alpha$.}
% % \vspace{-0.5em}
% \label{Fig: Demo AURC}
% \end{figure}

==> Figure-Tex/SVM-Figure-DisShift-2.tex <==
\begin{figure}[!tb]
\centering
\begingroup
\begin{tabular}{cc}
\centering
\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Dis-Shift-2/RC-Curves.png}
&\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Dis-Shift-2/Decision-Boundary.png}
\\
{\textbf{(a)} RC curves}
&{\textbf{(b)} Decision boundaries}
% \\
% \includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Geo-Margin.png}
% &\includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Max-SR.png}
% \\
% {\textbf{(c)} $s_{\text{geo}}$}
% &{\textbf{(d)} $s_{\text{sr}}$}
% % \\
% \includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Entropy.png}
% &\includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Max-Logit.png}
% \\
% {\textbf{(e)} $s_{\text{h}}$}
% &{\textbf{(f)} $s_{\text{ml}}$}
\end{tabular}
\endgroup 
% \caption{SC performance of the SVM classifier with different confidence scores under distribution shifts. Here, we can see that the rejection pattern of $s_{\text{geo}}$ benefits its RC performance over $s_{\text{sr}}$, $s_{\text{ml}}$, and $s_{\text{h}}$, and is even slightly better than $s_{\text{post}}$ which uses the posterior probability of the unshifted Gaussian distributions.}
\caption{SC performance using different selection confidence scores on the example SVM classifier under distribution shifts (Case 3). Here, the variance are larger than Case 1 --- classes are more inseparable and the samples are denser near the intersection center of all classes. From \textbf{(a)}, we can observer that (i) the base classifier performs poorly at full coverage (with selective risk $\sim 0.5$) and (ii) $s_{\text{geo}}$ is slightly worse than $s_{\text{sr}}$ in this case.}
\vspace{-0.5em}
\label{Fig: SVM Rejected Points Dist-shifts 2}
\end{figure}

==> Figure-Tex/SVM-Figure-DisShift.tex <==
\begin{figure}[!tb]
\centering
\begingroup
\begin{tabular}{cc}
\centering
\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Dis-Shift/RC-Curves.png}
&\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Dis-Shift/Radius-Remained.png}
\\
{\textbf{(a)} RC curves}
&{\textbf{(b)} Radius - Remained}
\\
\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Geo-Margin.png}
&\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Max-SR.png}
\\
{\textbf{(c)} $s_{\text{geo}}$}
&{\textbf{(d)} $s_{\text{sr}}$}
% \\
% \includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Entropy.png}
% &\includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Dis-Shift/Rejected-Points-Max-Logit.png}
% \\
% {\textbf{(e)} $s_{\text{h}}$}
% &{\textbf{(f)} $s_{\text{ml}}$}
\end{tabular}
\endgroup 
% \caption{SC performance of the SVM classifier with different confidence scores under distribution shifts. Here, we can see that the rejection pattern of $s_{\text{geo}}$ benefits its RC performance over $s_{\text{sr}}$, $s_{\text{ml}}$, and $s_{\text{h}}$, and is even slightly better than $s_{\text{post}}$ which uses the posterior probability of the unshifted Gaussian distributions.}
\caption{SC performance using different selection confidence scores on the example SVM classifier under distribution shifts (Case 2). Here, the samples are sparser near the intersection center of all classes. We see that the rejection pattern of $s_{\text{geo}}$ benefits its RC performance over $s_{\text{sr}}$, and is even slightly better than $s_{\text{post}}$ which uses the posterior probability of the unshifted Gaussian distributions.}
\vspace{-0.5em}
\label{Fig: SVM Rejected Points Dist-shifts}
\end{figure}

==> Figure-Tex/SVM-Figure-Heatmaps.tex <==
\begin{figure}[!tb]
\centering
\begingroup 
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{c c c c}
\centering

\includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/Heatmap-Geo-Margin.png}
&\includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/Heatmap-Max-SR.png}
&\includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/Heatmap-Entropy.png}
&\includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/Heatmap-Max-Logit.png}
\\
{\textbf{(a)} $s_{\text{geo}}$}
&{\textbf{(b)} $s_{\text{sr}}$}
&{\textbf{(c)} $s_{\text{h}}$}
&{\textbf{(d)} $s_{\text{ml}}$}

\end{tabular}
\endgroup 
\caption{Heat maps of different selective confidence scores on the input space (SVM classifier) --- \textbf{(a)} $s_{\text{geo}}$, \textbf{(b)} $s_{\text{sr}}$, \textbf{(c)} $s_{\text{h}}$ and \textbf{(d)} $s_{\text{ml}}$.  Within each subfigure, the darker the area, the lower the scores, the higher priority the selective classifiers (when paired with each selective confidence) to reject samples from. Unlike $s_{\text{sr}}$, $s_{\text{h}}$ and $s_{\text{ml}}$ where selective classifiers prioritize rejecting samples closer to the intersection of all classes, selective classifiers paired with $s_{\text{geo}}$ prioritize rejecting samples closer to the decision boundaries.}
\vspace{-0.5em}
\label{Fig: Selective Confidence Heatmaps}
\end{figure}

==> Figure-Tex/SVM-Figure-Rejected-Points.tex <==
% \begin{figure*}[!tb]
% \centering
% \begingroup 
% \setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{0.8}

% \begin{tabular}{c c c}
% \centering
% \includegraphics[width=0.28\textwidth]{Figures/SVM-Figures/RC-Curves.png}
% &\includegraphics[width=0.28\textwidth]{Figures/SVM-Figures/Radius-Rejects.png}
% &\includegraphics[width=0.28\textwidth]{Figures/SVM-Figures/Radius-Remained.png}
% \\
% {\textbf{(a)} RC curves}
% &{\textbf{(b)} Radius - Rejected}
% &{\textbf{(c)} Radius - Remained}
% \end{tabular}

% \begin{tabular}{c c c c}
% \centering
% \includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Rejected-Points-Geo-Margin.png}
% &\includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Rejected-Points-Max-SR.png}
% &\includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Rejected-Points-Entropy.png}
% &\includegraphics[width=0.18\textwidth]{Figures/SVM-Figures/Rejected-Points-Max-Logit.png}
% \\
% {\textbf{(d)} $s_{\text{geo}}$}
% &{\textbf{(r)} $s_{\text{sr}}$}
% &{\textbf{(f)} $s_{\text{h}}$}
% &{\textbf{(g)} $s_{\text{ml}}$}

% \end{tabular}
% \endgroup 
% \caption{SC performance of the SVM classifer using different selection confidence scores, where \textbf{(a)} is the RC curves achieved; \textbf{(b)-(g)} are visualization of sample rejection patterns of each selection confidence scores (plotted at $0.8$ coverage). In particular, \textbf{(b) \& (c)} are the histograms of the samples rejected and kept, respectively, where the x-axis is the distance to the closest decision boundary; \textbf{(d) - (g)} are the visualization of the rejected samples (black) and remained samples (orange, blue, red, and green, representing different class labels); and the dashed blue lines are the SVM decision boundaries.}
% \vspace{-0.5em}
% \label{Fig: SVM Rejected Points}
% \end{figure*}

\begin{figure}[!tb]
\centering
\begingroup
\begin{tabular}{cc}
\centering
\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/RC-Curves.png}
&\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Radius-Remained.png}
\\
{\textbf{(a)} RC curves}
&{\textbf{(b)} Radius - Remained}
\\
\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Rejected-Points-Geo-Margin.png}
&\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Rejected-Points-Max-SR.png}
\\
{\textbf{(c)} $s_{\text{geo}}$}
&{\textbf{(d)} $s_{\text{sr}}$}
\\
\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Rejected-Points-Entropy.png}
&\includegraphics[width=0.215\textwidth]{Figures/SVM-Figures/Rejected-Points-Max-Logit.png}
\\
{\textbf{(e)} $s_{\text{h}}$}
&{\textbf{(f)} $s_{\text{ml}}$}
\end{tabular}
\endgroup 
\caption{SC performance using different selection confidence scores on the example SVM classifier (Case 1). Here, \textbf{(a)} is the RC curves achieved; \textbf{(b)-(f)} are visualization of sample rejection patterns of each selection confidence scores (plotted at $0.8$ coverage). In particular, \textbf{(b)} are the histograms of the remaining $80 \%$ samples, where the x-axis is the distance to the closest decision boundary; \textbf{(c) - (f)} are the visualization of the rejected samples (black) and remaining samples (orange, blue, red, and green, representing different class labels); and the dashed blue lines are the SVM decision boundaries.}
\vspace{-0.5em}
\label{Fig: SVM Rejected Points}
\end{figure}

==> Figure-Tex/SVM-Figure-Samples-RC.tex <==
% \begin{figure}[!tb]
% \centering
% \begingroup 
% \setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{0.8}
% \begin{tabular}{c c c c}
% \centering

% \includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/Decision-Boundary.png}
% &\includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/RC-Curves.png}
% &\includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/Decision-Boundary.png}
% &\includegraphics[width=0.24\textwidth]{Figures/SVM-Figures/Decision-Boundary.png}
% \\
% {\textbf{(a)} xxx}
% &{\textbf{(b)} xxx}
% &{\textbf{(c)} xxx}
% &{\textbf{(d)} xxx}

% \end{tabular}
% \endgroup 
% \caption{xxxx }

% \label{Fig: xxx}
% \end{figure}

\begin{figure}[!tb]
\vspace{-2em}
\begin{tabular}{@{}cc@{}}
    \subfloat[Visualization of samples and the decision boundaries of SVM.]{%
        \label{a}%
        \includegraphics[width=0.36\textwidth]{Figures/SVM-Figures/Decision-Boundary.png}%
    }&
    \subfloat[RC curves.]{%
        \label{b}%
        \includegraphics[width=0.36\textwidth]{Figures/SVM-Figures/RC-Curves.png}%
    }
\end{tabular}\hfill
\begin{minipage}{0.21\textwidth}
\vspace{1.5em}
\caption{Visualization of \textbf{(a)} the four Gaussian distributions (each with $500$ sampled data points) and decision boundary achieved by the proposed SVM classifier and \textbf{(b)} the SC performance of using different selective confidence scores.}
\label{Fig: Vis SVM samples and RC curves}
\end{minipage}
\vspace{-0.5em}
\end{figure}

==> Table-Tex/AURC-A-Cifar-New.tex <==
\begin{table*}[!tb]
\caption{AURC-$\alpha$ summary of the SC performance using different confidence scores of CIFAR-10 and CIFAR-10-C experiments. All CIFAR-10-C corruptions are of severity $3$ in this table. The AURC numbers are \emph{on the $10^{-2}$ scale --- the lower, the better}. Gray background highlights scores computed on \emph{raw output logits}. The best AURC numbers for each coverage are highlighted in bold, and the second best are underlined.}
\label{tab: Partial AURC-A CIFAR}
\centering
\resizebox{1\linewidth}{!}{%
\begin{tabular}{l ccc c ccc c ccc c ccc c ccc}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{CIFAR-10} & & \multicolumn{3}{c}{Gaussian Blur} & & \multicolumn{3}{c}{Brightness} & & \multicolumn{3}{c}{Fog} & & \multicolumn{3}{c}{Snow}\\
\midrule
\multicolumn{1}{c}{\small{$\alpha$}} & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1\\
\toprule
\rowcolor{Gray}
$RL_{\text{conf-M}}$ & \textbf{0} & \textbf{0.013} & \textbf{0.242} & & \underline{0.05} & \underline{0.26} & \underline{1.74} & & \textbf{0} & \underline{0.05} & \underline{0.42} & & \textbf{0.12} & 0.42 & 2.52 & & \textbf{0} & \underline{0.17} & 1.47\\
\rowcolor{Gray}
$RL_{\text{geo-M}}$ & \underline{0.03} & 0.039 & 0.256 & & 0.16 & \textbf{0.24} & \textbf{1.70} & & 0.09 & 0.06 & \underline{0.42} & & 0.17 & \textbf{0.34} & \textbf{2.43} & & \underline{0.13} & \underline{0.17} & 1.49\\
\hdashline
\rowcolor{Gray}
$RL_{\text{max}}$ & \textbf{0} & 0.055 & 0.382 & & \textbf{0.04} & 0.43 & 2.02 & & \underline{0.01} & 0.08 & 0.58 & & \underline{0.41} & 0.60 & 2.73 & & \textbf{0} & 0.30 & 1.70\\

$SR_{\text{max}}$ & \textbf{0} & \underline{0.014} & \underline{0.244} & & 0.07 & \underline{0.26} & \underline{1.74} & & \textbf{0} & \textbf{0.04} & \textbf{0.41} & & 0.15 & \underline{0.41} & 2.50 & & \textbf{0} & \textbf{0.16} & \underline{1.45}\\
$SR_{\text{ent}}$ & \textbf{0} & \underline{0.014} & 0.245 & & 0.07 & 0.27 & \underline{1.74} & & \textbf{0} & \textbf{0.04} & \textbf{0.41} & & \underline{0.14} & \underline{0.41} & \underline{2.49} & & \textbf{0} & \textbf{0.16} & \textbf{1.44}\\
$SR_{\text{doctor}}$ & \textbf{0} & \underline{0.014} & \underline{0.244} & & 0.07 &
 \underline{0.26} & \underline{1.74} & & \textbf{0} & \textbf{0.04} & \textbf{0.41} & & 0.15 & \underline{0.41} & \underline{2.49} & & \textbf{0} & \textbf{0.16} & \underline{1.45}\\

% \midrule
% \rowcolor{Gray}
% $RL_{\text{conf-M}}$ & \textbf{0.12} & 0.91 & 4.34 & & \textbf{0} & \textbf{0.01} & \underline{0.93} & & \underline{0.01} & \underline{0.26} & \underline{1.71} & & 0.21 & \underline{0.38} & 2.59 & & \underline{0.04} & 0.28 & 1.66\\
% \rowcolor{Gray}
% $RL_{\text{geo-M}}$ & 0.23 & \textbf{0.77} & \textbf{4.22} & & 0.09 & \underline{0.10} & \textbf{0.92} & & 0.22 & \textbf{0.25} & \textbf{1.70} & & 0.42 & \underline{0.38} & 2.58 & & 0.23 & \underline{0.25} & \underline{1.65}\\
% \hdashline
% \rowcolor{Gray}
% $RL_{\text{max}}$ & 0.17 & 1.05 & 4.51 & & 0.08 & 0.20 & 1.16 & & 0.08 & 0.46 & 2.01 & & \textbf{0.10} & 0.47 & 2.71 & & 0.08 & 0.32 & 1.86\\

% $SR_{\text{max}}$ & \underline{0.14} & \underline{0.87} & 4.29 & & \underline{0.01} & \underline{0.10} & \underline{0.93} & & \textbf{0} & 0.27 & \underline{1.71} & & \underline{0.13} & \textbf{0.35} & 2.56 & & \textbf{0} & \textbf{0.23} & \textbf{1.63}\\
% $SR_{\text{ent}}$ & \underline{0.14} & \underline{0.87} & \underline{4.27} & & 0.02 & \underline{0.10} & \underline{0.93} & & \textbf{0} & 0.28 & 1.72 & & \underline{0.13} & \textbf{0.35} & \textbf{2.54} & & \textbf{0} & \textbf{0.23} & \textbf{1.63}\\
% $SR_{\text{doctor}}$ & \underline{0.14} & \underline{0.87} & 4.28 & & \underline{0.01} & \underline{0.10} & \underline{0.93} & & \textbf{0} & 0.27 & \underline{1.71} & & \underline{0.13} & \textbf{0.35} & \underline{2.55} & & \textbf{0} & \textbf{0.23} & \textbf{1.63}\\

% \midrule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Glass Blur} & & \multicolumn{3}{c}{Gaussian Noise} & & \multicolumn{3}{c}{Impulse Noise} & & \multicolumn{3}{c}{JPEG} & & \multicolumn{3}{c}{Speckle Noise}\\
% \midrule
% \rowcolor{Gray}
% $RL_{\text{conf-M}}$ & \textbf{0.39} & \underline{2.02} & 8.41 & & \underline{0.73} & 2.46 & 7.66 & & 0.12 & 1.40 & 6.93 & & \underline{0.29} & 0.79 & 3.84 & & 0.48 & \underline{0.51} & \underline{2.21}\\
% \rowcolor{Gray}
% $RL_{\text{geo-M}}$ & 0.52 & \textbf{1.98} & 8.43 & & \textbf{0.57} & \textbf{2.27} & 7.58 & & 0.08 & \textbf{1.08} & \textbf{6.63} & & 0.33 & \textbf{0.69} & \textbf{3.78} & & 0.53 & \textbf{0.49} & 2.24\\
% \hdashline
% \rowcolor{Gray}
% $RL_{\text{max}}$ & 0.70 & 2.55 & 8.64 & & 1.05 & 2.92 & 7.80 & & \textbf{0} & \underline{1.1} & \underline{6.64} & & \textbf{0.25} & 1.03 & 4.15 & & 0.51 & 0.87 & 2.56\\

% $SR_{\text{max}}$ & \underline{0.40} & 2.03 & 8.30 & & 0.83 & \underline{2.42} & 7.56 & & \underline{0.05} & 1.16 & 6.69 & & \underline{0.29} & \underline{0.75} & \underline{3.79} & & \underline{0.47} & 0.56 & \underline{2.21}\\
% $SR_{\text{ent}}$ & \underline{0.40} & 2.03 & \textbf{8.27} & & 0.84 & \underline{2.42} & \textbf{7.52} & & \underline{0.05} & 1.14 & 6.65 & & \underline{0.29} & \underline{0.75} & \underline{3.79} & & \textbf{0.46} & 0.56 & \textbf{2.20}\\
% $SR_{\text{doctor}}$ & \underline{0.40} & 2.03 & \underline{8.29} & & 0.82 & \underline{2.42} & \underline{7.54} & & \underline{0.05} & 1.16 & 6.67 & & 0.33 & 0.76 & \underline{3.79} & & \underline{0.47} & 0.56 & \textbf{2.20}\\

% \midrule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Motion Blur} & & \multicolumn{3}{c}{Pixelate} & & \multicolumn{3}{c}{Saturate} & & \multicolumn{3}{c}{Shot Noise} & & \multicolumn{3}{c}{Zoom Blur}\\
% \midrule
% \rowcolor{Gray}
% $RL_{\text{conf-M}}$ & \underline{0.15} & 1.08 & 5.26 & & \textbf{0} & \underline{0.11} & \underline{1.09} & & \textbf{0} & \underline{0.05} & \textbf{0.23} & & \underline{0.46} & \underline{0.96} & 3.73 & & \underline{0.01} & \underline{0.23} & 1.62\\
% \rowcolor{Gray}
% $RL_{\text{geo-M}}$ & \textbf{0.12} & \textbf{0.92} & \textbf{5.10} & & 0.11 & \textbf{0.10} & 1.10 & & \textbf{0} & 0.06 & \textbf{0.23} & & 0.48 & \textbf{0.90} & 3.74 & & 0.11 & \textbf{0.21} & \textbf{1.59}\\
% \hdashline
% \rowcolor{Gray}
% $RL_{\text{max}}$ & 0.23 & 1.27 & 5.49 & & \underline{0.02} & 0.27 & 1.33 & & \textbf{0} & 0.06 & \underline{0.33} & & 0.58 & 1.56 & 4.15 & & 0.06 & 0.36 & 1.86\\

% $SR_{\text{max}}$ & 0.17 & \underline{1.03} & 5.19 & & \textbf{0} & \underline{0.11} & \textbf{1.08} & & \textbf{0} & \textbf{0.04} & \textbf{0.23} & & \underline{0.46} & 1.00 & \underline{3.72} & & \textbf{0} & \textbf{0.21} & \underline{1.61}\\
% $SR_{\text{ent}}$ & 0.17 & \underline{1.03} & \underline{5.18} & & \textbf{0} & \underline{0.11} & \textbf{1.08} & & \textbf{0} & \textbf{0.04} & \textbf{0.23} & & \textbf{0.45} & 1.01 & \textbf{3.71} & & \textbf{0} & \textbf{0.21} & \underline{1.61}\\
% $SR_{\text{doctor}}$ & 0.17 & \underline{1.03} & \underline{5.18} & & \textbf{0} & \underline{0.11} & \textbf{1.08} & & \textbf{0} & \textbf{0.04} & \textbf{0.23} & & \underline{0.46} & 1.00 & \textbf{3.71} & & \textbf{0} & \textbf{0.21} & \underline{1.61}
% \\
\bottomrule
\end{tabular}}%
\vspace{-0.5em}
\end{table*}%



==> Table-Tex/AURC-A-Cifar.tex <==
\begin{table*}[!tb]
\caption{AURC-$\alpha$ summary of the SC performance comparison with SCnet. All CIFAR-10-C corruptions are of severity $3$ in this table. The number of AURCs are \emph{on the $10^{-2}$ scale.} Scores in gray shade are the nontraining based. The best AURC values at each coverage are highlighted in bold, and the second best are underscored.}
\label{tab: Partial AURC-A CIFAR (SCnet)}
\centering
\resizebox{1\linewidth}{!}{%
\begin{tabular}{l ccc c ccc c ccc c ccc c ccc}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{CIFAR-10} & & \multicolumn{3}{c}{Gaussian Blur} & & \multicolumn{3}{c}{Brightness} & & \multicolumn{3}{c}{Fog} & & \multicolumn{3}{c}{Snow}\\
\midrule
\multicolumn{1}{c}{\small{$\alpha$}} & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1\\
\toprule
\rowcolor{Gray}
$RL_{\text{conf-M}}$  & 0.10 & 0.28 & 1.04 & & \textbf{0.57} & \underline{1.85} & \underline{8.56} & & 0.15 & 0.35 & 1.28 & & 0.38 & 0.64 & 2.51 & & 0.58 & 1.11 & 4.77\\
\rowcolor{Gray}
$RL_{\text{geo-M}}$ & \textbf{0} & \textbf{0.19} & \textbf{0.96} & & 1.00 & 2.09 & 8.93 & & \textbf{0.01} & \underline{0.29} & \textbf{1.21} & & \textbf{0.13} & \textbf{0.48} & \textbf{2.43} & & \textbf{0.47} & \underline{1.02} & \textbf{4.67}\\
\hdashline
\rowcolor{Gray}
$RL_{\text{max}}$  & 1.01 & 1.03 & 1.56 & & 1.87 & 2.39 & 8.60 & & 0.82 & 0.92 & 1.69 & & 1.02 & 1.20 & 2.82 & & 1.58 & 2.08 & 5.33\\
\rowcolor{Gray}
$SR_{\text{max}}$  & 0.83 & 0.82 & 1.41 & & 1.69 & 2.27 & 8.65 & & 0.66 & 0.81 & 1.59 & & 0.87 & 1.09 & 2.75 & & 1.48 & 1.85 & 5.19\\
\rowcolor{Gray}
$SR_{\text{ent}}$  & 0.87 & 0.84 & 1.42 & & 1.72 & 2.28 & 8.62 & & 0.68 & 0.82 & 1.60 & & 0.89 & 1.10 & 2.75 & & 1.50 & 1.88 & 5.20\\
\rowcolor{Gray}
$SR_{\text{doctor}}$  & 0.83 & 0.82 & 1.41 & & 1.70 & 2.27 & 8.64 & & 0.66 & 0.81 & 1.59 & & 0.87 & 1.09 & 2.75 & & 1.48 & 1.85 & 5.19\\
SCnet  & \underline{0.07} & \underline{0.23} & \underline{1.01} & & \underline{0.85} & \textbf{1.74} & \textbf{8.16} & & \underline{0.07} & \textbf{0.28} & \underline{1.24} & & \underline{0.28} & \underline{0.55} & \underline{2.47} & & \underline{0.49} & \textbf{0.94} & \underline{4.68}\\

% \midrule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Contrast} & & \multicolumn{3}{c}{Defocus Blur} & & \multicolumn{3}{c}{Elastic} & & \multicolumn{3}{c}{Frost} & & \multicolumn{3}{c}{Spatter}\\
% \midrule
% \rowcolor{Gray}
% $RL_{\text{conf-M}}$ & 1.29 & 1.87 & 7.31 & & 0.31 & 0.55 & \underline{3.22} & & \textbf{0.19} & \underline{0.71} & \underline{4.13} & & \textbf{0.48} & 1.77 & 7.66 & & \underline{0.20} & \underline{0.90} & 4.38\\
% \rowcolor{Gray}
% $RL_{\text{geo-M}}$ & \textbf{0.88} & \textbf{1.51} & \textbf{7.22} & & \textbf{0.09} & \underline{0.51} & 3.28 & & 0.26 & \underline{0.71} & 4.23 & & \textbf{0.48} & \underline{1.68} & \underline{7.62} & & 0.35 & 0.92 & \underline{4.34}\\
% \hdashline
% \rowcolor{Gray}
% $RL_{\text{max}}$ & 2.63 & 2.68 & 7.56 & & 0.78 & 1.01 & 3.43 & & 1.23 & 1.35 & 4.38 & & 1.49 & 2.85 & 8.17 & & 0.96 & 1.81 & 4.91\\
% \rowcolor{Gray}
% $SR_{\text{max}}$ & 2.39 & 2.48 & 7.53 & & 0.60 & 0.86 & 3.36 & & 1.03 & 1.18 & 4.32 & & 1.44 & 2.56 & 8.04 & & 0.76 & 1.54 & 4.74\\
% \rowcolor{Gray}
% $SR_{\text{ent}}$ & 2.42 & 2.50 & 7.51 & & 0.61 & 0.88 & 3.36 & & 1.05 & 1.20 & 4.32 & & 1.45 & 2.59 & 8.04 & & 0.78 & 1.57 & 4.75\\
% \rowcolor{Gray}
% $SR_{\text{doctor}}$ & 2.39 & 2.48 & 7.52 & & 0.60 & 0.86 & 3.36 & & 1.03 & 1.18 & 4.32 & & 1.44 & 2.56 & 8.03 & & 0.76 & 1.54 & 4.74\\
% SCnet & \underline{1.06} & \underline{1.76} & \underline{7.23} & & \underline{0.18} & \textbf{0.48} & \textbf{3.08} & & \underline{0.22} & \textbf{0.65} & \textbf{3.98} & & \underline{0.67} & \textbf{1.50} & \textbf{7.37} & & \textbf{0.10} & \textbf{0.65} & \textbf{4.26}\\

% \midrule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Glass Blur} & & \multicolumn{3}{c}{Gaussian Noise} & & \multicolumn{3}{c}{Impulse Noise} & & \multicolumn{3}{c}{JPEG} & & \multicolumn{3}{c}{Speckle Noise}\\
% \midrule
% \rowcolor{Gray}
% $RL_{\text{conf-M}}$ & \underline{2.34} & \underline{7.79} & \underline{17.6} & & \underline{12.6} & \underline{22.8} & \underline{32.8} & & 1.61 & \underline{3.49} & \underline{10.5} & & \underline{1.13} & 1.23 & 4.06 & & \underline{2.31} & \underline{4.52} & \underline{12.0}\\
% \rowcolor{Gray}
% $RL_{\text{geo-M}}$ & 3.15 & 7.98 & 17.7 & & 16.3 & 23.4 & 33.1 & & \underline{1.53} & 3.61 & \underline{10.5} & & \textbf{0.62} & \textbf{1.06} & \textbf{3.96} & & 3.83 & 4.94 & 12.1\\
% \hdashline
% \rowcolor{Gray}
% $RL_{\text{max}}$ & 5.41 & 9.57 & 18.4 & & 19.8 & 27.4 & 35.0 & & 2.57 & 4.36 & 10.9 & & 1.34 & 1.97 & 4.46 & & 4.85 & 6.80 & 13.1\\
% \rowcolor{Gray}
% $SR_{\text{max}}$ & 4.81 & 9.13 & 18.2 & & 18.0 & 26.3 & 34.6 & & 2.31 & 4.05 & 10.7 & & 1.24 & 1.77 & 4.35 & & 4.36 & 6.22 & 12.8\\
% \rowcolor{Gray}
% $SR_{\text{ent}}$ & 4.88 & 9.19 & 18.2 & & 19.0 & 26.4 & 34.6 & & 2.34 & 4.08 & 10.7 & & 1.26 & 1.79 & 4.35 & & 4.43 & 6.28 & 12.8\\
% \rowcolor{Gray}
% $SR_{\text{doctor}}$ & 4.81 & 9.13 & 18.2 & & 18.9 & 26.3 & 34.5 & & 2.31 & 4.05 & 10.7 & & 1.24 & 1.77 & 4.34 & & 4.36 & 6.22 & 12.8\\
% SCnet & \textbf{1.00} & \textbf{6.86} & \textbf{17.1} & & \textbf{2.15} & \textbf{16.5} & \textbf{29.1} & & \textbf{0.99} & \textbf{2.61} & \textbf{10.0} & & 1.36 & \underline{1.20} & \underline{4.00} & & \textbf{0.54} & \textbf{2.73} & \textbf{10.8}\\

% \midrule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Motion Blur} & & \multicolumn{3}{c}{Pixelate} & & \multicolumn{3}{c}{Saturate} & & \multicolumn{3}{c}{Shot Noise} & & \multicolumn{3}{c}{Zoom Blur}\\
% \midrule
% \rowcolor{Gray}
% $RL_{\text{conf-M}}$ & \underline{1.34} & \underline{3.27} & \underline{11.5} & & 1.11 & 1.15 & 3.51 & & 0.14 & 0.32 & \underline{1.10} & & \underline{3.64} & \underline{9.03} & \underline{18.5} & & \textbf{0.52} & \underline{1.59} & 8.20\\
% \rowcolor{Gray}
% $RL_{\text{geo-M}}$ & 1.43 & 3.37 & 11.7 & & \textbf{0.50} & \textbf{0.84} & \textbf{3.27} & & \textbf{0} & \textbf{0.24} & \textbf{1.02} & & 5.66 & 9.59 & 18.7 & & 0.93 & 1.85 & 8.58\\
% \hdashline
% \rowcolor{Gray}
% $RL_{\text{max}}$ & 3.43 & 4.06 & 11.6 & & 2.43 & 2.68 & 4.44 & & 1.41 & 0.99 & 1.57 & & 6.91 & 12.2 & 20.0 & & 0.59 & 1.71 & \underline{8.03}\\
% \rowcolor{Gray}
% $SR_{\text{max}}$ & 3.02 & 3.82 & 11.6 & & 2.10 & 2.34 & 4.21 & & 1.16 & 0.85 & 1.45 & & 6.53 & 11.4 & 19.6 & & \underline{0.57} & 1.65 & 8.11\\
% \rowcolor{Gray}
% $SR_{\text{ent}}$ & 3.06 & 3.85 & 11.6 & & 2.15 & 2.37 & 4.23 & & 1.19 & 0.86 & 1.46 & & 6.59 & 11.5 & 19.7 & & \underline{0.57} & 1.66 & 8.08\\
% \rowcolor{Gray}
% $SR_{\text{doctor}}$ & 3.02 & 3.82 & 11.6 & & 2.10 & 2.38 & 4.20 & & 1.16 & 0.85 & 1.45 & & 6.53 & 11.4 & 19.6 & & \underline{0.57} & 1.65 & 8.11\\
% SCnet & \textbf{0.99} & \textbf{3.03} & \textbf{11.2} & & \underline{0.63} & \underline{1.01} & \underline{3.50} & & \underline{0.11} & \underline{0.28} & \underline{1.10} & & \textbf{0.44} & \textbf{5.93} & \textbf{16.5} & & 0.77 & \textbf{1.41} & \textbf{7.87}\\
\bottomrule
\end{tabular}}%
\end{table*}%

==> Table-Tex/AURC-training-based-score.tex <==
\begin{table*}[!tb]

\caption{Training-based scores}
\label{tab: traing-based-score}
\centering

\resizebox{1\linewidth}{!}{%
\begin{tabular}{l ccc c ccc c ccc c ccc}
\multicolumn{1}{c}{} & \multicolumn{3}
{c}{\small{In-D (ImageNet)}} & & \multicolumn{3}{c}{\small{In-D + Shift (Cov)}} & & \multicolumn{3}{c}{\small{In-D + Shift (Label)}} &
 & \multicolumn{3}{c}{\small{In-D + Shift (both)}}\\
\midrule
\multicolumn{1}{c}{\small{$\alpha$}} & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1 & & 0.1 & 0.5 & 1\\
\toprule
\rowcolor{Gray}
$RL_{\text{conf-M}}$ & \textbf{0.16} & \textbf{0.53} & \textbf{2.39} & & \textbf{0.24} & \textbf{0.96} & \textbf{4.77} & & \textbf{1.04} & \underline{3.34} & \underline{11.7} & & \textbf{0.34} & \textbf{1.20} & \textbf{5.43}\\
\rowcolor{Gray}
$RL_{\text{geo-M}}$ & \underline{0.27} & \underline{0.59} & \underline{2.43} & & \underline{0.37} & \underline{1.02} & \underline{4.78} & & \underline{1.20} & \underline{3.35} & \underline{11.6} & & \underline{0.48} & \underline{1.26} & \textbf{5.43}\\
\hdashline
\rowcolor{Gray}
SIRC & 2.23 & \underline{2.07} & \underline{3.36} & & 3.71 & 3.06 & \underline{5.83} & & 15.8 & 8.88 & 13.7 & & 4.61 & 3.53 & 6.52\\
\rowcolor{Gray}
$SR_{\text{max}}$ & 3.20 & 2.36 & 3.38 & & 4.52 & 3.66 & 5.93 & & 13.1 & 7.52 & 12.6 & & 5.21 & 3.75 & 6.56\\

\rowcolor{Gray}
$SR_{\text{ent}}$ & 4.28 & 3.13 & 4.04 & & 6.24 & 4.66 & 7.00 & & 16.0 & 9.19 & 13.4 & & 7.04 & 5.10 & 7.61\\
\rowcolor{Gray}
$SR_{\text{doctor}}$ & 3.22 & 2.38 & 3.40 & & 4.55 & 3.40 & 6.00 & & 13.2 & 7.55 & 12.6 & & 5.24 & 3.78 & 6.61\\

$RL_{\text{max}}$ & 5.53 & 4.05 & 4.57 & & 8.48 & 6.04 & 7.64 & & 21.1 & 11.9 & 14.9 & & 9.53 & 6.59 & 8.33\\
Energy & 8.13 & 6.60 & 6.90 & & 12.8 & 10.3 & 11.1 & & 27.3 & 16.6 & 18.1 & & 14.1 & 11.0 & 11.8\\
KNN & \underline{0.99} & 2.27 & 4.58 & & \underline{1.22} & \underline{2.89} & 6.78 & & \underline{1.18} & \textbf{3.23} & \textbf{10.8} & & \underline{1.24} & \underline{2.98} & \underline{7.16}\\
ViM & 5.48 & 7.11 & 8.31 & & 5.31 & 8.05 & 10.4 & & 5.83 & 7.89 & 13.4 & & 5.35 & 8.12 & 10.7\\
\bottomrule
\end{tabular}}
\end{table*}%
